Continual Learning of Diffusion Models with Generative Distillation

Diffusion models are powerful generative models that achieve state-of-the-art performance in image synthesis. However, training them demands substantial amounts of data and computational resources. Continual learning would allow for incrementally learning new tasks and accumulating knowledge, thus enabling the reuse of trained models for further learning. One potentially suitable continual learning approach is generative replay, where a copy of a generative model trained on previous tasks produces synthetic data that are interleaved with data from the current task. However, standard generative replay applied to diffusion models results in a catastrophic loss in denoising capabilities. In this paper, we propose generative distillation, an approach that distils the entire reverse process of a diffusion model. We demonstrate that our approach substantially improves the continual learning performance of generative replay with only a modest increase in the computational costs.

==> sections/old_experiments.tex <==


\section{OLD EXPERIMENTS SECTION}

\subsection{Experimental setup} 
We divide the Fashion-MNIST and CIFAR-10 datasets into five tasks, each comprising two randomly selected classes (\cref{fig:task_order}), that must be learned one after the other. To generate replay samples for previous tasks, we use the previous task model~$\epsilon_{\hat{\theta}_{i-1}}$ with 2 DDIM steps on Fashion-MNIST and 10 DDIM steps on CIFAR-10 for both generative replay and generative distillation. In Fashion-MNIST, we use a variation of the U-Net architecture used for CIFAR-10 in \citet{ho2020denoising} (refer to \cref{appendix:models_diffusion} for details) and, in CIFAR-10, we use the same architecture without any modifications.

To quantitatively compare the trained diffusion models, we report the commonly used Fréchet Inception Distance~(FID)~\citep{heusel2017gans}. We also report the Kullback-Leibler divergence between the ground truth class frequency distribution and the distribution of predicted class membership for images generated by the diffusion model. This last metric, denoted KLD, evaluates to what extent the diffusion model generates samples from all classes so far (rather than, for example, only from classes of the last task). To compute this metric, we use a ResNet18~\citep{he2015deep} trained on each of the datasets. The models are evaluated only on the test subset comprising all the classes seen so far after training on each task. When generating replay samples to train the continually trained classifier and when computing the evaluation metrics, we use 10 DDIM steps on Fashion-MNIST and 20 DDIM steps on CIFAR-10. 

For each metric, we include baselines that can be interpreted as upper and lower targets. The upper target is attained through joint training of either the classifier or the diffusion model, wherein we sequentially train the models using all the data from tasks encountered so far. The lower target is obtained by naïvely fine-tuning the models on the current task. The upper target yields desirable metrics, while the lower target serves as a performance baseline.

For further details on the experiment, models and metrics, please refer to \cref{appendix:extra_details}.

% Due to limited computational resources, we stop the training at each task before the model converges, thus leading to poorer image quality. 

\subsection{Generative distillation}
The results in \cref{tab:results_cl_gen} and \cref{tab:results_cl_gen_cifar} indicate a severe loss in denoising capabilities when using standard generative replay on both datasets. As shown in \cref{fig:results_qualitative_gr} and \cref{fig:results_qualitative_cifar}, after training on the last tasks, the generative replay trained model generates images that are too smooth, indicating that the model quickly forgets how to add detail to the images. 
%Increasing the number of DDIM steps when generating the replay samples would increase computational costs and the accumulation of error would still present, albeit less prominent (see \cref{appendix:extra_experiments_results} and \cref{fig:qualitative_gr10}). 
On the other hand, generative distillation preserves previous knowledge much more effectively and the model still generates high-quality and detailed images (\cref{fig:results_qualitative_gd}), while using the same computational budget plus one extra forward pass. The performance of generative replay can be improved by increasing the number of DDIM steps when generating the replay samples, but generative distillation clearly outperforms generative replay in all settings we consider on both datasets (\cref{appendix:extra_experiments_results} and \cref{fig:qualitative_gr10,fig:qualitative_gd10,fig:qualitative_gr100,fig:qualitative_gd100}). 

% I remove this line since it may be due to the underfitting.
% Interestingly, the FID of the generative distillation trained model slightly improved from tasks 2 to 4 (\cref{fig:results_cl_metrics_through_tasks}), which may indicate positive transfer between tasks. 


%% EXAMPLE OF HOW THE RESULTS OF F-MNIST AND CIFAR CAN BE MERGED
\begin{table}
    \centering
    \caption{\label{tab:results_cl_gen}\textbf{Generative distillation.} The FID and KLD are computed after training on all tasks. Reported for each metric is mean ± standard error over 3 random seeds.}
    \begin{tabular}{llllll}
\toprule
& \multicolumn{2}{c}{\bf Fashion MNIST} & & \multicolumn{2}{c}{\bf CIFAR-10} \\
Strategy & ~~~~$\downarrow \text{FID}$ & ~~$\downarrow \text{KLD}$ & & ~~~~$\downarrow \text{FID}$ & ~~$\downarrow \text{KLD}$ \\
\midrule
    Joint \scriptsize{(upper target)} & ~~15.5 \scriptsize{$\pm$ 1.3} & 0.08 \scriptsize{$\pm$ 0.02} & & 31.9 \scriptsize{$\pm$ 2.9} & 0.12 \scriptsize{$\pm$ 0.02}\\
    Finetune \scriptsize{(lower target)} & ~~68.8 \scriptsize{$\pm$ 7.0} & 4.82 \scriptsize{$\pm$ 1.42} & & 55.8 \scriptsize{$\pm$ 2.6} & 1.14 \scriptsize{$\pm$ 0.10}\\
    \midrule
    Generative replay & 211.8 \scriptsize{$\pm$ 6.9} & 3.39 \scriptsize{$\pm$ 0.30} & & 96.4 \scriptsize{$\pm$ 5.3} & 0.74 \scriptsize{$\pm$ 0.14}\\
    Generative distillation & ~~\textbf{23.5 \scriptsize{$\pm$ 1.1}} & \textbf{0.25 \scriptsize{$\pm$ 0.10}} & & \textbf{42.3 \scriptsize{$\pm$ 4.7}} & \textbf{0.16 \scriptsize{$\pm$ 0.01}} \\
    \bottomrule  
\end{tabular}
\end{table}

\begin{figure}
\centering
\begin{subfigure}[b]{0.25\textwidth}
     \centering
     \includegraphics[width=\linewidth]{assets/experiment/incremental_classes.drawio.pdf}
     \caption{Task order}
     \label{fig:task_order}
\end{subfigure}
\hspace{0.05\textwidth}
\begin{subfigure}[b]{0.223\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/experiment/joint_samples.png}
     \caption{Joint}
\end{subfigure}
%\hspace{0.01\textwidth}
\begin{subfigure}[b]{0.223\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/experiment/gr2_samples.png}
     \caption{GR}
     \label{fig:results_qualitative_gr}
\end{subfigure}
\begin{subfigure}[b]{0.223\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/experiment/gd2_samples.png}
     \caption{GD}
     \label{fig:results_qualitative_gd}
\end{subfigure}
\caption{\textbf{Qualitative results on Fashion-MNIST.} (a)~The order of the tasks the models were trained on. (b-d)~Images generated at the end of training by a diffusion model that was jointly trained on all tasks, continually trained using generative replay (GR) or continually trained using generative distillation (GD). When introducing distillation into generative replay, the model keeps its denoising capabilities and diversity.}
\label{fig:results_qualitative}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.471\textwidth}
         \centering
         \includegraphics{assets/experiment/stream_fid_comparison.pdf}
         %\caption{$\text{avg }FID$ throughout tasks}
         %\label{fig:results_cl_fid}
     \end{subfigure}
     \qquad
     \begin{subfigure}[b]{0.471\textwidth}
         \centering
         \includegraphics{assets/experiment/stream_kld_comparison.pdf}
         %\caption{$\text{avg }KLD$ throughout tasks}
         %\label{fig:results_cl_kld}
     \end{subfigure}
    \caption{\textbf{Quality of the diffusion model throughout the continual learning process on Fashion-MNIST.} For each approach, the FID and KLD of the diffusion model are computed after every task. Displayed are the means ± standard errors over 3 random seeds. Joint: training using data from all tasks so far (upper target), Naive: continual fine-tuning (lower target), GR: generative replay, GD: generative distillation.}
    \label{fig:results_cl_metrics_through_tasks}
\end{figure}
 

\begin{figure}
\centering
\begin{subfigure}[b]{0.25\textwidth}
     \centering
     \includegraphics[width=\linewidth]{assets/experiment/cifar10/incremental_classes.drawio.pdf}
     \caption{Task order}
     \label{fig:task_order_cifar}
\end{subfigure}
\hspace{0.05\textwidth}
\begin{subfigure}[b]{0.223\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/experiment/cifar10/joint_samples.png}
     \caption{Joint}
\end{subfigure}
%\hspace{0.01\textwidth}
\begin{subfigure}[b]{0.223\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/experiment/cifar10/gr10_samples.png}
     \caption{GR}
     \label{fig:results_qualitative_gr_cifar}
\end{subfigure}
\begin{subfigure}[b]{0.223\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/experiment/cifar10/gd10_samples.png}
     \caption{GD}
     \label{fig:results_qualitative_gd_cifar}
\end{subfigure}
\caption{\textbf{Qualitative results on CIFAR-10.} (a)~The order of the tasks the models were trained on. (b-d)~Images generated at the end of training by a diffusion model that was jointly trained on all tasks, continually trained using generative replay (GR) or continually trained using generative distillation (GD). Introducing distillation into generative replay prevents the catastrophic accumulation of error and the model is still able to produce detailed images.}
\label{fig:results_qualitative_cifar}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.471\textwidth}
         \centering
         \includegraphics{assets/experiment/cifar10/stream_fid_comparison.pdf}
         %\caption{$\text{avg }FID$ throughout tasks}
         %\label{fig:results_cl_fid}
     \end{subfigure}
     \qquad
     \begin{subfigure}[b]{0.471\textwidth}
         \centering
         \includegraphics{assets/experiment/cifar10/stream_kld_comparison.pdf}
         %\caption{$\text{avg }KLD$ throughout tasks}
         %\label{fig:results_cl_kld}
     \end{subfigure}
    \caption{\textbf{Quality of the diffusion model throughout the continual learning process on CIFAR-10.} For each approach, the FID and KLD of the diffusion model are computed after every task. Displayed are the means ± standard errors over 3 random seeds. Joint: training using data from all tasks so far (upper target), Naive: continual fine-tuning (lower target), GR: generative replay, GD: generative distillation.}
    \label{fig:results_cl_metrics_through_tasks_cifar}
\end{figure}




\subsection{Using the diffusion model for training a classifier with generative replay}
As an additional way of evaluating the performance of the continually trained diffusion model, we include a classifier trained with generative replay using the continually trained diffusion model as generator (see \cref{appendix:cont_class} for details). In Tables \ref{tab:results_cl_clf} and \ref{tab:results_cl_clf_cifar}, we report the accuracy of the classifier at the end of training for both Fashion-MNIST and CIFAR-10. This evaluation confirms the benefit of incorporating distillation into generative replay.

\begin{table}
    \centering
    \caption{\textbf{Evaluation with a continually trained classifier.} Reported is mean ± standard error over 3~seeds.}\label{tab:results_cl_clf}
    \small
    \begin{tabular}{lcc}
        \toprule
        & \textbf{Fashion-MNIST} & \textbf{CIFAR-10} \\
        Strategy & $\uparrow \text{ACC}$ & $\uparrow \text{ACC}$ \\
        \midrule
        Joint \it \scriptsize{(upper target)} & 0.92\scriptsize{ $\pm$ 0.00} & 0.77\scriptsize{ $\pm$ 0.03} \\
        Finetune \it \scriptsize{(lower target)} & 0.17\scriptsize{ $\pm$ 0.03} & 0.19\scriptsize{ $\pm$ 0.00} \\
        \midrule
        Generative replay & 0.50\scriptsize{$\pm$ 0.04} & 0.27\scriptsize{$\pm$ 0.02} \\
        Generative distillation & \textbf{0.72\scriptsize{$\pm$ 0.03}} & \textbf{0.33 \scriptsize{$\pm$ 0.02}} \\
        \bottomrule
    \end{tabular}
\end{table}




\subsection{Alternative distillation approaches}
To further illustrate the potential of distillation, we provide an additional experiment in which the knowledge of the model from the previous task is distilled using the current task's data. This can be seen as a Learning without Forgetting~(LwF)~\citep{li2017learning} like approach applied to diffusion models. This approach exhibited better performance than naïve generative replay both in quality and diversity when the teacher used up to 10 DDIM steps. However, the overall quality of the samples degrades steadily and more artefacts show up as more tasks are learned.

We also considered an extreme case equivalent to the model from the previous task using 0 DDIM steps, that is, distilling with Gaussian noise as input for all timesteps. Surprisingly, this approach surpasses distillation with current data in FID. In contrast, it shows a worse KLD, indicating that distilling with noise sacrifices diversity over image quality. The reason for poorer diversity when using Gaussian noise might be that the noise doesn't align well with the actual distribution, whereas the lower quality obtained when distilling with current data could be attributed to conflicting gradients calculated in the loss function. Distilling with Gaussian noise achieves the second best ACC only behind generative distillation, which shows the potential of distillation for transferring knowledge even when employing only noise.





==> sections/preliminary.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.195\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/preliminary/0000.png}
     \caption{Task 1}
\end{subfigure}
\begin{subfigure}[b]{0.195\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/preliminary/0001.png}
     \caption{Task 2}
\end{subfigure}
\begin{subfigure}[b]{0.195\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/preliminary/0002.png}
     \caption{Task 3}
\end{subfigure}
\begin{subfigure}[b]{0.195\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/preliminary/0003.png}
     \caption{Task 4}
\end{subfigure}
\begin{subfigure}[b]{0.195\textwidth}
     \centering
     \includegraphics[width=\textwidth]{assets/preliminary/0004.png}
     \caption{Task 5}
\end{subfigure}
\caption{\textbf{Preliminary experiment qualitative results.} After the first task is learned, the model from the previous task generates replay samples for the current task model. Displayed are the images generated for seed 42. Naïve generative replay causes a catastrophic degradation of the denoising capabilities of the diffusion model in previous tasks.}
\label{fig:preliminaries_qualitative_cl}
\end{figure}

DDPM takes extended generation times, which makes continual training through generative replay extremely slow and limits the number of samples generated. Using DDIM is a solution that allows for sampling a greater amount of images. However, we conducted a preliminary experiment where it was shown that naïve generative replay alone is not enough to mitigate the phenomenon of catastrophic forgetting in diffusion models. We adopted a class-incremental approach, dividing the Fashion-MNIST dataset into 5 tasks, each consisting of two randomly selected classes. The diffusion model then learned these tasks sequentially through generative replay. To generate synthetic samples for training on previous tasks, the teacher used 2 DDIM steps, as this produced visually acceptable and distinguishable images. In spite of this, the results in \Cref{fig:preliminaries_qualitative_cl} clearly show a severe loss in denoising capabilities for previous tasks. One solution would involve increasing the number of teacher DDIM steps, although this comes at higher computation costs. Moreover, the accumulation of error is still present, albeit less prominent. In this paper, we explore an alternative approach based on knowledge distillation that mitigates this catastrophic loss in denoising capabilities without increasing the number of teacher DDIM steps.

==> sections/related_work_old.tex <==
\paragraph{Diffusion models} Diffusion models are likelihood-based models~\citep{song2020generative, ho2020denoising, song2021scorebased} defined by two processes: (1)~a forward process that adds Gaussian noise to an image according to a variance schedule and (2)~a learnable reverse process that follows the reverse trajectory of the forward process. The forward and reverse processes are discretized into $T$ timesteps. A diffusion model, denoted as $\epsilon_\theta$ and parameterized by $\theta$, can be trained to match the noise introduced during the forward process at any timestep~$t$ following a predefined variance schedule. To train this model, one can minimize the following simplified objective~\citep{ho2020denoising}: 
\begin{equation}\label{eq:gr_loss_generator_simple}
    L_\text{simple}(\theta) = \mathbb{E}_{t \sim \text{Unif}(T), x_0 \sim D, \epsilon \sim \mathcal{N}(0, I)} \bigr[ 
        \|\epsilon - \epsilon_\theta(\sqrt{\alpha_t}x_0+\sqrt{1-\alpha_t}\epsilon, t)\|^2
    \bigr],
\end{equation}
where $x_0$ is a clean sample from the data distribution $D$, $\epsilon \sim \mathcal{N}(0, I)$ is the ground truth Gaussian noise, and $\alpha$ is variance schedule function. The standard way of sampling from a diffusion model (e.g., with DDPM) is computationally expensive as it requires many denoising steps (e.g., 1000 in \citet{ho2020denoising}). This greatly limits the number of samples that can be generated for replay with a finite computational budget. One widely used alternative is DDIM~\citep{song2020denoising}, which makes the forward process non-Markovian and introduces a stochastic parameter $\sigma$ that, when set to zero, makes the sampling processes deterministic. DDIM permits sampling using a smaller number of denoising steps, thus allowing the generation of more images given the same computational budget. However, the fewer denoising steps are used, the blurrier and less detailed the sampled images tend to be. Each denoising step from $t \in T$ to $s \in T$ such that $s < t$ of DDIM runs
\begin{equation}\label{eq:ddim_sampling}
    x_{s} = \sqrt{\alpha_{s}} \biggl(\frac{x_t - \sqrt{1-\alpha_t}\epsilon_\theta(x_t)}{\sqrt{\alpha_t}} \biggr) 
     + \sqrt{1-\alpha_{s}-\sigma_t^2} \cdot \epsilon_\theta(x_t)
     + \sigma_t \epsilon.
 \end{equation} 
where $\sigma_t$ is the parameter that controls the stochasticity.

\paragraph{Knowledge distillation in diffusion models} Existing studies use distillation in diffusion models to train a student such that it can generate the same quality images as its teacher, but in fewer generation steps~\citep{luhman2021knowledge, salimans2022progressive, berthelot2023tract, song2023consistency, gu2023boot}. In this paper, we use this technique for a different purpose and we demonstrate its effectiveness for continual learning of diffusion models.

\paragraph{Continual learning} An important problem in continual learning is catastrophic forgetting~\citep{MCCLOSKEY1989109, Ratcliff1990ConnectionistMO}, a phenomenon where a sequentially trained neural network rapidly and drastically forgets its knowledge of previous tasks when it learns a new task. Current approaches that aim to mitigate catastrophic forgetting can be categorized as architectural or parameter isolation methods, regularization methods and rehearsal methods~\citep{biesialska-etal-2020-continual, survey_cl}. Architectural methods~\citep{rusu2016progressive, yoon2017lifelong, Scardapane_2017, Masse_2018, wortsman2020supermasks, activedendrite} prevent interference by introducing new modules or by using a fixed set of parameters for each task. Regularization methods~\citep{Kirkpatrick_2017, synapticintel, ahn2019uncertaintybased, li2017learning} preserve the knowledge from previous tasks through the addition of extra terms to the loss function. Rehearsal methods~\citep{Ratcliff1990ConnectionistMO, rehearsal1995, rebuffi2017icarl, lopezpaz2022gradient, chaudhry2019efficient} also known as \textit{experience replay}, use an episodic buffer to store all or a subset of the previous tasks' samples and replay them during the training of the subsequent tasks interlaced with real data from the current task. 

In some situations, there may be privacy issues or compute constraints that forbid storing any previous data. One approach to mitigate catastrophic forgetting under these circumstances is generative replay~\citep{shin2017}. Given a sequence of $B$ tasks $\mathcal{T}_i=\{\mathcal{T}_1, \mathcal{T}_2, ..., \mathcal{T}_B\}$, a generative model~$G_i$ is trained on data from task~$T_i$ interleaved with replay samples produced by $G_{i-1}$, a copy of the generative model after it finished training on the previous task.

In this work, we work under the assumption that the architecture of the model will not vary throughout the continual training process and that we do not have access to previous data. Therefore, we use the generative replay framework to explain our methods.

\paragraph{Continual learning and diffusion models} The topic of continual learning of diffusion models remains relatively unexplored. We are aware of three works that use generative replay in diffusion models. \citet{zajac2023exploring} test different continual learning approaches on diffusion models, and \citet{gao2023ddgr} use a continually trained classifier to guide the generation process, as in \citep{dhariwal2021diffusion}. These works, however, do not study the use of DDIM in generative replay. In other recent work, \citet{smith2023continual} observe a catastrophic accumulation of errors when using standard generative replay.


